Search for $C\!P$ violation in $D^+_{(s)}\to{}K_{S}^{0}K^{-}\pi^{+}\pi^{+}$ decays using triple and quadruple products

We perform the first search for $C\!P$ violation in ${D_{(s)}^{+}\to{}K_{S}^{0}K^{-}\pi^{+}\pi^{+}}$ decays. We use a combined data set from the Belle and Belle II experiments, which study $e^+e^-$ collisions at center-of-mass energies at or near the $\Upsilon(4S)$ resonance. We use 980 fb$^{-1}$ of data from Belle and 428 fb$^{-1}$ of data from Belle~II. We measure six $C\!P$-violating asymmetries that are based on triple products and quadruple products of the momenta of final-state particles, and also the particles' helicity angles. We obtain a precision at the level of 0.5% for $D^+\to{}K_{S}^{0}K^{-}\pi^{+}\pi^{+}$ decays, and better than 0.3% for $D^+_{s}\to{}K_{S}^{0}K^{-}\pi^{+}\pi^{+}$ decays. No evidence of $C\!P$ violation is found. Our results for the triple-product asymmetries are the most precise to date for singly-Cabibbo-suppressed $D^+$ decays. Our results for the other asymmetries are the first such measurements performed for charm decays.

==> belle2-symbols.tex <==
% Standard Belle II aliases
% A. Di Canto (16-Sep-2022)
% Based on:
%  - babarsym.tex (by D. Hitlin, D. MacFarlane, P. Dauncey, R. Waldi)
%  - lhcb-symbols-def.tex (by U. Egede, T. Skwarnicki, C. Parkes, R. Oldeman, P. Koppenburg)

\RequirePackage{xspace}
\RequirePackage{relsize}

%%%%%%%%%%%%%
% Experiments
%%%%%%%%%%%%%
\def\belletwo{\mbox{Belle~II}\xspace}
\def\belle  {\mbox{Belle}\xspace}
\def\lhcb {\mbox{LHCb}\xspace}
%\def\babar  {\mbox{BaBar}\xspace}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}\xspace}

%%%%%%%%%%%%%
% Particles
%%%%%%%%%%%%%
\def\Palpha      {\ensuremath{\alpha}\xspace}
\def\Pbeta       {\ensuremath{\beta}\xspace}
\def\Pgamma      {\ensuremath{\gamma}\xspace}                 
\def\Pdelta      {\ensuremath{\delta}\xspace}                 
\def\Pepsilon    {\ensuremath{\epsilon}\xspace}                 
\def\Pvarepsilon {\ensuremath{\varepsilon}\xspace}                 
\def\Pzeta       {\ensuremath{\zeta}\xspace}                 
\def\Peta        {\ensuremath{\eta}\xspace}                 
\def\Ptheta      {\ensuremath{\theta}\xspace}                 
\def\Pvartheta   {\ensuremath{\vartheta}\xspace}                 
\def\Piota       {\ensuremath{\iota}\xspace}                 
\def\Pkappa      {\ensuremath{\kappa}\xspace}                 
\def\Plambda     {\ensuremath{\lambda}\xspace}                 
\def\Pmu         {\ensuremath{\mu}\xspace}                 
\def\Pnu         {\ensuremath{\nu}\xspace}                 
\def\Pxi         {\ensuremath{\xi}\xspace}                 
\def\Ppi         {\ensuremath{\pi}\xspace}                 
\def\Pvarpi      {\ensuremath{\varpi}\xspace}                 
\def\Prho        {\ensuremath{\rho}\xspace}                 
\def\Pvarrho     {\ensuremath{\varrho}\xspace}                 
\def\Ptau        {\ensuremath{\tau}\xspace}                 
\def\Pupsilon    {\ensuremath{\upsilon}\xspace}                 
\def\Pphi        {\ensuremath{\phi}\xspace}                 
\def\Pvarphi     {\ensuremath{\varphi}\xspace}                 
\def\Pchi        {\ensuremath{\chi}\xspace}                 
\def\Ppsi        {\ensuremath{\psi}\xspace}                 
\def\Pomega      {\ensuremath{\omega}\xspace}                 
\mathchardef\PDelta="7101
\mathchardef\PXi="7104
\mathchardef\PLambda="7103
\mathchardef\PSigma="7106
\mathchardef\POmega="710A
\mathchardef\PUpsilon="7107
\def\PA      {\ensuremath{A}\xspace}                 
\def\PB      {\ensuremath{B}\xspace}                 
\def\PC      {\ensuremath{C}\xspace}                 
\def\PD      {\ensuremath{D}\xspace}                 
\def\PE      {\ensuremath{E}\xspace}                 
\def\PF      {\ensuremath{F}\xspace}                 
\def\PG      {\ensuremath{G}\xspace}                 
\def\PH      {\ensuremath{H}\xspace}                 
\def\PI      {\ensuremath{I}\xspace}                 
\def\PJ      {\ensuremath{J}\xspace}                 
\def\PK      {\ensuremath{K}\xspace}                 
\def\PL      {\ensuremath{L}\xspace}                 
\def\PM      {\ensuremath{M}\xspace}                 
\def\PN      {\ensuremath{N}\xspace}                 
\def\PO      {\ensuremath{O}\xspace}                 
\def\PP      {\ensuremath{P}\xspace}                 
\def\PQ      {\ensuremath{Q}\xspace}                 
\def\PR      {\ensuremath{R}\xspace}                 
\def\PS      {\ensuremath{S}\xspace}                 
\def\PT      {\ensuremath{T}\xspace}                 
\def\PU      {\ensuremath{U}\xspace}                 
\def\PV      {\ensuremath{V}\xspace}                 
\def\PW      {\ensuremath{W}\xspace}                 
\def\PX      {\ensuremath{X}\xspace}                 
\def\PY      {\ensuremath{Y}\xspace}                 
\def\PZ      {\ensuremath{Z}\xspace}                 
\def\Pa      {\ensuremath{a}\xspace}                 
\def\Pb      {\ensuremath{b}\xspace}                 
\def\Pc      {\ensuremath{c}\xspace}                 
\def\Pd      {\ensuremath{d}\xspace}                 
\def\Pe      {\ensuremath{e}\xspace}                 
\def\Pf      {\ensuremath{f}\xspace}                 
\def\Pg      {\ensuremath{g}\xspace}                 
\def\Ph      {\ensuremath{h}\xspace}                 
\def\Pi      {\ensuremath{i}\xspace}                 
\def\Pj      {\ensuremath{j}\xspace}                 
\def\Pk      {\ensuremath{k}\xspace}                 
\def\Pl      {\ensuremath{l}\xspace}                 
\def\Pm      {\ensuremath{m}\xspace}                 
\def\Pn      {\ensuremath{n}\xspace}                 
\def\Po      {\ensuremath{o}\xspace}                 
\def\Pp      {\ensuremath{p}\xspace}                 
\def\Pq      {\ensuremath{q}\xspace}                 
\def\Pr      {\ensuremath{r}\xspace}                 
\def\Ps      {\ensuremath{s}\xspace}                 
\def\Pt      {\ensuremath{t}\xspace}                 
\def\Pu      {\ensuremath{u}\xspace}                 
\def\Pv      {\ensuremath{v}\xspace}                 
\def\Pw      {\ensuremath{w}\xspace}                 
\def\Px      {\ensuremath{x}\xspace}                 
\def\Py      {\ensuremath{y}\xspace}                 
\def\Pz      {\ensuremath{z}\xspace}                 

%% generic

\def\hpm  {\ensuremath{\Ph^\pm}\xspace} 
\def\hp     {\ensuremath{\Ph^+}\xspace} 
\def\hm    {\ensuremath{\Ph^-}\xspace}
\def\ellpm{\ensuremath{\ell^\pm}\xspace}
\def\ellp   {\ensuremath{\ell^+}\xspace}
\def\ellm  {\ensuremath{\ell^-}\xspace}

%% Leptons

\let\emi\en
\def\electron   {\ensuremath{\Pe}\xspace}
\def\en         {\ensuremath{\Pe^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{\Pe^+}\xspace}
\def\epm        {\ensuremath{\Pe^\pm}\xspace} 
\def\epem       {\ensuremath{\Pe^+\Pe^-}\xspace}
\def\ee         {\ensuremath{\Pe^-\Pe^-}\xspace}

\def\mmu        {\ensuremath{\Pmu}\xspace}
\def\mup        {\ensuremath{\Pmu^+}\xspace}
\def\mun        {\ensuremath{\Pmu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\Pmu^+\Pmu^-}\xspace}
\def\mtau       {\ensuremath{\Ptau}\xspace}

\def\taup       {\ensuremath{\Ptau^+}\xspace}
\def\taum       {\ensuremath{\Ptau^-}\xspace}
\def\tautau     {\ensuremath{\Ptau^+\Ptau^-}\xspace}

\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\neu        {\ensuremath{\Pnu}\xspace}
\def\neub       {\ensuremath{\overline{\Pnu}}\xspace}
\def\nuenueb    {\ensuremath{\neu\neub}\xspace}
\def\neue       {\ensuremath{\neu_e}\xspace}
\def\neueb      {\ensuremath{\neub_e}\xspace}
\def\neueneueb  {\ensuremath{\neue\neueb}\xspace}
\def\neum       {\ensuremath{\neu_\mu}\xspace}
\def\neumb      {\ensuremath{\neub_\mu}\xspace}
\def\neumneumb  {\ensuremath{\neum\neumb}\xspace}
\def\neut       {\ensuremath{\neu_\tau}\xspace}
\def\neutb      {\ensuremath{\neub_\tau}\xspace}
\def\neutneutb  {\ensuremath{\neut\neutb}\xspace}
\def\neul       {\ensuremath{\neu_\ell}\xspace}
\def\neulb      {\ensuremath{\neub_\ell}\xspace}
\def\neulneulb  {\ensuremath{\neul\neulb}\xspace}

%% Gauge bosons and scalars

\def\g      {\ensuremath{\Pgamma}\xspace}
\def\H      {\ensuremath{\PH^0}\xspace}
\def\Hp     {\ensuremath{\PH^+}\xspace}
\def\Hm     {\ensuremath{\PH^-}\xspace}
\def\Hpm    {\ensuremath{\PH^\pm}\xspace}
\def\W      {\ensuremath{\PW}\xspace}
\def\Wp     {\ensuremath{\PW^+}\xspace}
\def\Wm     {\ensuremath{\PW^-}\xspace}
\def\Wpm    {\ensuremath{\PW^\pm}\xspace}
\def\Z      {\ensuremath{\PZ^0}\xspace}

%% Quarks

\def\quark     {\ensuremath{\Pq}\xspace}
\def\quarkbar  {\ensuremath{\overline \quark}\xspace}
\def\qqbar     {\ensuremath{\quark\quarkbar}\xspace}
\def\uquark    {\ensuremath{\Pu}\xspace}
\def\uquarkbar {\ensuremath{\overline \uquark}\xspace}
\def\uubar     {\ensuremath{\uquark\uquarkbar}\xspace}
\def\dquark    {\ensuremath{\Pd}\xspace}
\def\dquarkbar {\ensuremath{\overline \dquark}\xspace}
\def\ddbar     {\ensuremath{\dquark\dquarkbar}\xspace}
\def\squark    {\ensuremath{\Ps}\xspace}
\def\squarkbar {\ensuremath{\overline \squark}\xspace}
\def\ssbar     {\ensuremath{\squark\squarkbar}\xspace}
\def\cquark    {\ensuremath{\Pc}\xspace}
\def\cquarkbar {\ensuremath{\overline \cquark}\xspace}
\def\ccbar     {\ensuremath{\cquark\cquarkbar}\xspace}
\def\bquark    {\ensuremath{\Pb}\xspace}
\def\bquarkbar {\ensuremath{\overline \bquark}\xspace}
\def\bbbar     {\ensuremath{\bquark\bquarkbar}\xspace}
\def\tquark    {\ensuremath{\Pt}\xspace}
\def\tquarkbar {\ensuremath{\overline \tquark}\xspace}
\def\ttbar     {\ensuremath{\tquark\tquarkbar}\xspace}

%% Light mesons

\def\pion  {\ensuremath{\Ppi}\xspace}
\def\piz   {\ensuremath{\pion^0}\xspace}
\def\pizs  {\ensuremath{\pion^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pion^0\pion^0}\xspace}
\def\pip   {\ensuremath{\pion^+}\xspace}
\def\pim   {\ensuremath{\pion^-}\xspace}
\def\pipi  {\ensuremath{\pion^+\pion^-}\xspace}
\def\pipm  {\ensuremath{\pion^\pm}\xspace}
\def\pimp  {\ensuremath{\pion^\mp}\xspace}
\def\pisoft{\ensuremath{\pion_s}\xspace}
\def\kaon  {\ensuremath{\PK}\xspace}
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em \PK}{}\xspace}% do NOT use ensuremath here
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{\kaon^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{\kaon^+}\xspace}
\def\Km    {\ensuremath{\kaon^-}\xspace}
\def\Kpm   {\ensuremath{\kaon^\pm}\xspace}
\def\Kmp   {\ensuremath{\kaon^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{\kaon^0_S}\xspace} 
\def\KL    {\ensuremath{\kaon^0_L}\xspace} 
\def\Kstarz  {\ensuremath{\kaon^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{\kaon^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{\kaon^{*+}}\xspace}
\def\Kstarm  {\ensuremath{\kaon^{*-}}\xspace}
\def\Kstarpm {\ensuremath{\kaon^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{\kaon^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\Peta^{\prime}}\xspace}

%% Heavy mesons

\def\D       {\ensuremath{\PD}\xspace}
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em \PD}{}\xspace}% do NOT use ensuremath here
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{\D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{\D^+}\xspace}
\def\Dm      {\ensuremath{\D^-}\xspace}
\def\Dpm     {\ensuremath{\D^\pm}\xspace}
\def\Dmp     {\ensuremath{\D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{\D^*}\xspace}
\def\Dsttt   {\ensuremath{\Dstar(2010)^+}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{\D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{\D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{\D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{\D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{\D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{\D^+_\squark}\xspace}
\def\Dsp     {\ensuremath{\D^+_\squark}\xspace}
\def\Dsm     {\ensuremath{\D^-_\squark}\xspace}
\def\Dspm    {\ensuremath{\D^{\pm}_\squark}\xspace}
\def\Dsmp    {\ensuremath{\D^{\mp}_\squark}\xspace}
\def\Dss     {\ensuremath{\D^{*+}_\squark}\xspace}
\def\Dssp    {\ensuremath{\D^{*+}_\squark}\xspace}
\def\Dssm    {\ensuremath{\D^{*-}_\squark}\xspace}
\def\Dsspm   {\ensuremath{\D^{*\pm}_\squark}\xspace}
\def\Dssmp   {\ensuremath{\D^{*\mp}_\squark}\xspace}

\def\B       {\ensuremath{\PB}\xspace}
\def\Bbar    {\ensuremath{\kern 0.18em\overline{\kern -0.18em \PB}{}}\xspace}% do NOT use ensuremath here
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BBbar   {\ensuremath{\B\Bbar}\xspace} 
\def\Bz      {\ensuremath{\B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\Bu      {\ensuremath{\B^+}\xspace}
\def\Bub     {\ensuremath{\B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{\B^\pm}\xspace}
\def\Bmp     {\ensuremath{\B^\mp}\xspace}
\def\Bd      {\ensuremath{\B^0}\xspace}
\def\Bs      {\ensuremath{\B^0_\squark}\xspace}
\def\Bsb     {\ensuremath{\Bbar^0_\squark}\xspace}
\def\Bdb     {\ensuremath{\Bbar^0}\xspace}
\def\Bc      {\ensuremath{\B_\cquark^+}\xspace}
\def\Bcp     {\ensuremath{\B_\cquark^+}\xspace}
\def\Bcm     {\ensuremath{\B_\cquark^-}\xspace}
\def\Bcpm    {\ensuremath{\B_\cquark^\pm}\xspace}

%% Onia

\def\jpsi     {\ensuremath{{\PJ\mskip -3mu/\mskip -2mu\Ppsi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\Ppsi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\Ppsi(3770)}\xspace}
\def\etac     {\ensuremath{\Peta_\cquark}\xspace}
\def\chiczero {\ensuremath{\Pchi_{\cquark 0}}\xspace}
\def\chicone  {\ensuremath{\Pchi_{\cquark 1}}\xspace}
\def\chictwo  {\ensuremath{\Pchi_{\cquark 2}}\xspace}
\def\Y#1S{\ensuremath{\PUpsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

\def\chic  {\ensuremath{\Pchi_{c}}\xspace}

%% Baryons

\def\proton      {\ensuremath{\Pp}\xspace}
\def\antiproton  {\ensuremath{\overline \proton}\xspace}
\def\neutron     {\ensuremath{\Pn}\xspace}
\def\antineutron {\ensuremath{\overline \neutron}\xspace}

\def\Deltares {\ensuremath{\PDelta}\xspace}
\def\Deltaresbar{\ensuremath{\overline \Deltares}\xspace}
\def\Xires {\ensuremath{\PXi}\xspace}
\def\Xiresbar{\ensuremath{\overline \Xires}\xspace}
\def\L {\ensuremath{\PLambda}\xspace}
\def\Lbar {\ensuremath{\kern 0.1em\overline{\kern -0.1em\PLambda}}\xspace}
\def\Lambdares {\ensuremath{\PLambda}\xspace}
\def\Lambdaresbar{\ensuremath{\Lbar}\xspace}
\def\Sigmares {\ensuremath{\PSigma}\xspace}
\def\Sigmaresbar{\ensuremath{\overline \Sigmares}\xspace}
\def\Omegares {\ensuremath{\POmega}\xspace}
\def\Omegaresbar{\ensuremath{\overline \Omegares}\xspace}

\def\Lz      {\ensuremath{\L^0}\xspace}
\def\Lzbar   {\ensuremath{\Lbar^0}\xspace}
\def\Lc      {\ensuremath{\L^+_\cquark}\xspace}
\def\Lcbar   {\ensuremath{\Lbar^-_\cquark}\xspace}
\def\Lb      {\ensuremath{\L^0_\bquark}\xspace}
\def\Lbbar   {\ensuremath{\Lbar^0_\bquark}\xspace}

%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%

%% Decays
\def\BF         {{\ensuremath{\cal B}\xspace}}
\def\BRvis      {{\ensuremath{\BR_{\rm{vis}}}}}
\def\BR         {\BF}
\newcommand{\decay}[2]{\ensuremath{#1\!\to #2}\xspace}         % {\Pa}{\Pb \Pc}
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

%% EW theory, groups
\def\grpsuthree {\ensuremath{\mathrm{SU}(3)}\xspace}
\def\grpsutw    {\ensuremath{\mathrm{SU}(2)}\xspace}
\def\grpuone    {\ensuremath{\mathrm{U}(1)}\xspace}

\def\ssqtw {\ensuremath{\sin^{2}\!\theta_{\mathrm{W}}}\xspace}
\def\csqtw {\ensuremath{\cos^{2}\!\theta_{\mathrm{W}}}\xspace}
\def\stw   {\ensuremath{\sin\theta_{\mathrm{W}}}\xspace}
\def\ctw   {\ensuremath{\cos\theta_{\mathrm{W}}}\xspace}
\def\ssqtwef {\ensuremath{{\sin}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}\xspace}
\def\csqtwef {\ensuremath{{\cos}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}\xspace}
\def\stwef {\ensuremath{\sin\theta_{\mathrm{W}}^{\mathrm{eff}}}\xspace}
\def\ctwef {\ensuremath{\cos\theta_{\mathrm{W}}^{\mathrm{eff}}}\xspace}
\def\gv    {\ensuremath{g_{\mbox{\tiny V}}}\xspace}
\def\ga    {\ensuremath{g_{\mbox{\tiny A}}}\xspace}

\def\order   {\ensuremath{\mathcal{O}}\xspace}
\def\ordalph {\ensuremath{\mathcal{O}(\alpha)}\xspace}
\def\ordalsq {\ensuremath{\mathcal{O}(\alpha^{2})}\xspace}
\def\ordalcb {\ensuremath{\mathcal{O}(\alpha^{3})}\xspace}

%% QCD parameters
\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}
\def\qsq       {\ensuremath{q^2}\xspace}

%% CKM, CP violation

\def\eps   {\ensuremath{\varepsilon}\xspace}
\def\epsK  {\ensuremath{\varepsilon_K}\xspace}
\def\epsB  {\ensuremath{\varepsilon_B}\xspace}
\def\epsp  {\ensuremath{\varepsilon^\prime_K}\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace}
\def\CPV               {\ensuremath{C\!PV}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}

\def\Vud  {\ensuremath{|V_{\uquark\dquark}|}\xspace}
\def\Vcd  {\ensuremath{|V_{\cquark\dquark}|}\xspace}
\def\Vtd  {\ensuremath{|V_{\tquark\dquark}|}\xspace}
\def\Vus  {\ensuremath{|V_{\uquark\squark}|}\xspace}
\def\Vcs  {\ensuremath{|V_{\cquark\squark}|}\xspace}
\def\Vts  {\ensuremath{|V_{\tquark\squark}|}\xspace}
\def\Vub  {\ensuremath{|V_{\uquark\bquark}|}\xspace}
\def\Vcb  {\ensuremath{|V_{\cquark\bquark}|}\xspace}
\def\Vtb  {\ensuremath{|V_{\tquark\bquark}|}\xspace}

%% Oscillations

\newcommand{\dm}{\ensuremath{\Delta m}\xspace}
\newcommand{\dms}{\ensuremath{\Delta m_{\squark}}\xspace}
\newcommand{\dmd}{\ensuremath{\Delta m_{\dquark}}\xspace}
\newcommand{\DG}{\ensuremath{\Delta\Gamma}\xspace}
\newcommand{\DGs}{\ensuremath{\Delta\Gamma_{\squark}}\xspace}
\newcommand{\DGd}{\ensuremath{\Delta\Gamma_{\dquark}}\xspace}
\newcommand{\Gs}{\ensuremath{\Gamma_{\squark}}\xspace}
\newcommand{\Gd}{\ensuremath{\Gamma_{\dquark}}\xspace}

\newcommand{\MBq}{\ensuremath{M_{\B_\quark}}\xspace}
\newcommand{\DGq}{\ensuremath{\Delta\Gamma_{\quark}}\xspace}
\newcommand{\Gq}{\ensuremath{\Gamma_{\quark}}\xspace}
\newcommand{\dmq}{\ensuremath{\Delta m_{\quark}}\xspace}
\newcommand{\GL}{\ensuremath{\Gamma_{\rm L}}\xspace}
\newcommand{\GH}{\ensuremath{\Gamma_{\rm H}}\xspace}

\newcommand{\ACP}{\ensuremath{{\cal A}^{\CP}}\xspace}
\newcommand{\Adir}{\ensuremath{{\cal A}^{\rm dir}}\xspace}
\newcommand{\Amix}{\ensuremath{{\cal A}^{\rm mix}}\xspace}
\newcommand{\ADelta}{\ensuremath{{\cal A}^\Delta}\xspace}

%% Tagging
\newcommand{\eff}{{\ensuremath{\varepsilon}}\xspace}
\newcommand{\efftag}{{\ensuremath{\varepsilon_{\rm tag}}}\xspace}
\newcommand{\mistag}{\ensuremath{\omega}\xspace}
\newcommand{\effeff}{{\ensuremath{\varepsilon_{\rm eff}}}\xspace}
\newcommand{\efftageff}{{\ensuremath{\varepsilon^{\rm eff}_{\rm tag}}}\xspace}

%%% QM
%\newcommand{\bra}[1]{\ensuremath{\langle #1|}}             % {a}
%\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}              % {b}
%\newcommand{\braket}[2]{\ensuremath{\langle #1|#2\rangle}} % {a}{b}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Units
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\unit}[1]{\ensuremath{\rm\,#1}\xspace}          % {kg}

%% Energy and momentum
\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
%\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\gevgevcccc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^4}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}

%% Distance and area
\def\km   {\ensuremath{\rm \,km}\xspace}
\def\m    {\ensuremath{\rm \,m}\xspace}
\def\cm   {\ensuremath{\rm \,cm}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{\rm \,mm}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{\,\upmu\rm m}\xspace}
\def\muma {\ensuremath{\,\upmu\rm m^2}\xspace}
\def\nm   {\ensuremath{\rm \,nm}\xspace}
\def\fm   {\ensuremath{\rm \,fm}\xspace}
\def\barn{\ensuremath{\rm \,b}\xspace}
\def\barnhyph{\ensuremath{\rm -b}\xspace}
\def\mbarn{\ensuremath{\rm \,mb}\xspace}
\def\mub{\ensuremath{\rm \,\upmu b}\xspace}
\def\mbarnhyph{\ensuremath{\rm -mb}\xspace}
\def\nb {\ensuremath{\rm \,nb}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{\rm \,pb}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\ab   {\ensuremath{\mbox{\,ab}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}

%% Time 
\def\sec  {\ensuremath{\rm {\,s}}\xspace}
\def\ms   {\ensuremath{{\rm \,ms}}\xspace}
\def\mus  {\ensuremath{\,\upmu{\rm s}}\xspace}
\def\ns   {\ensuremath{{\rm \,ns}}\xspace}
\def\ps   {\ensuremath{{\rm \,ps}}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}

\def\mhz  {\ensuremath{{\rm \,MHz}}\xspace}
\def\khz  {\ensuremath{{\rm \,kHz}}\xspace}
\def\hz   {\ensuremath{{\rm \,Hz}}\xspace}

\def\invps{\ensuremath{{\rm \,ps^{-1}}}\xspace}

\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}

%% Temperature
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}

%% Angles
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}
\def\rad{\ensuremath{\rm \,rad}\xspace}

%% Material lengths, radiation
\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\def\mip {MIP\xspace}
\def\neutroneq {\ensuremath{\rm \,n_{eq}}\xspace}
\def\neqcmcm {\ensuremath{\rm \,n_{eq} / cm^2}\xspace}
\def\kRad {\ensuremath{\rm \,kRad}\xspace}
\def\MRad {\ensuremath{\rm \,MRad}\xspace}
\def\ci {\ensuremath{\rm \,Ci}\xspace}
\def\mci {\ensuremath{\rm \,mCi}\xspace}

%% Uncertainties
\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}

%% Maths
\def\order{{\ensuremath{\cal O}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\chisqndf}{\ensuremath{\chisq/\mathrm{ndf}}\xspace}
\def\deriv {\ensuremath{\mathrm{d}}}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\newcommand{\mean}[1]{\ensuremath{\left\langle #1 \right\rangle}} % {x}
%\newcommand{\abs}[1]{\ensuremath{\left\|#1\right\|}} % {x}
\newcommand{\Real}{\ensuremath{\mathcal{R}e}\xspace}
\newcommand{\Imag}{\ensuremath{\mathcal{I}m}\xspace}

\def\sPlot{\mbox{\em sPlot}}
\def\sWeight{\mbox{\em sWeight}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Kinematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Energy, Momenta
\def\Ebeam {\ensuremath{E_{\mbox{\tiny BEAM}}}\xspace}
\def\sqs   {\ensuremath{\protect\sqrt{s}}\xspace}

\def\pt         {\mbox{$p_{\rm T}$}\xspace}
\def\et         {\mbox{$E_{\rm T}$}\xspace}

\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Programs
\def\evtgen   {\mbox{\textsc{EvtGen}}\xspace}
\def\pythia    {\mbox{\textsc{Pythia8}}\xspace}
\def\kkmc     {\mbox{\textsc{KKMC}}\xspace}
\def\geant     {\mbox{\textsc{Geant4}}\xspace}
\def\geantb     {\mbox{\textsc{Geant3}}\xspace}
\def\photos   {\mbox{\textsc{Photos}}\xspace}
\def\tauola    {\mbox{\textsc{TAUOLA}}\xspace}
\def\root       {\mbox{\textsc{Root}}\xspace}
\def\roofit     {\mbox{\textsc{RooFit}}\xspace}
\def\pyroot   {\mbox{\textsc{PyRoot}}\xspace}

%% Languages
\def\cpp        {\mbox{\textsc{C\raisebox{0.1em}{{\footnotesize{++}}}}}\xspace}
\def\python     {\mbox{\textsc{Python}}\xspace}
\def\ruby       {\mbox{\textsc{Ruby}}\xspace}
\def\fortran    {\mbox{\textsc{Fortran}}\xspace}

%%%%%%%%%%%%%%%
% Special Text 
%%%%%%%%%%%%%%%
\newcommand{\eg}{\mbox{\itshape e.g.}\xspace}
\newcommand{\ie}{\mbox{\itshape i.e.}}
\newcommand{\etal}{{\slshape et al.}\xspace}
\newcommand{\etc}{\mbox{\itshape etc.}\xspace}
\newcommand{\cf}{\mbox{\itshape cf.}\xspace}
\newcommand{\ffp}{\mbox{\itshape ff.}\xspace}
\newcommand{\vs}{\mbox{\itshape vs.}\xspace}


==> pub060.tex <==
%%% Paper:    D_s+ to KS0 K- pi+ pi+
%%% Journal:  JHEP
%%% Contacts: L.K. Li, A. Schwartz, K. Kinoshita
%%% ====================================================================
%%% Use \input{pub060} to insert this material into your latex file.
\newcounter{AffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCPPM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYerevan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGoettingen{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBeihang{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBNL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBINP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCMU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCinvestavIPN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPrague{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instChiangMai{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instChiba{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instChonnam{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instChula{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCAU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instConacyt{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instDESY{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instDuke{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instITAR{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFuJen{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFudan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGifu{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSOKENDAI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMainz{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGyeongsang{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHanyang{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instHeidelberg{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKEK{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJPARC{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instHiroshima{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHUNNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFrascati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNapoliINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPadovaINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPerugiaINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPisaINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRomaTreINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTorinoINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTriesteINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIISc{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIISER{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITBhubaneswar{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITGuwahati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITHyderabad{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instIITJodhpur{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITMadras{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIndiana{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIHEPRussia{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHEPHYVienna{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIHEPChina{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIPP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIOP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIFIC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instISU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJAEA{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJLU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKarlsruhe{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKitasato{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKISTI{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instKoreaUnivKU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instKSU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKyotoU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKyungpook{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLNNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGiessen{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLuther{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMNITJaipur{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLMU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMcGill{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNagoya{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNagoyaKMI{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instNNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNankai{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNaraWu{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instUNAM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHSE{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNTUTaiwan{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instNUUTaiwan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKrakow{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNiigata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNSU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instOsakaMetropolitan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRCNP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPNNL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPanjab{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instPeking{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMPP{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMPGHLL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPanjabPAU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRIKENMSL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instShandong{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKyiv{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSPU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSoochow{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSoongsil{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSEU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaJSI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSKKU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTUM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTelAviv{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instToho{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instTitech{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instTokyoMetropolitan{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instUAS{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNapoliUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPadovaUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPerugiaUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPisaUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRomaTreUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTorinoUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTriesteUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIJCLab{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIPHC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instAdelaide{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instUofA{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBonn{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUBC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCincinnati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFlorida{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHamburg{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHawaii{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaUniLJ{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLouisville{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMalaya{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instManitoba{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaUM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMelbourne{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMississippi{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instUOM{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instNovaGorica{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUPES{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPittsburgh{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUSTC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSAlabama{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instSCarolina{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSydney{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTabuk{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUTokyo{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instEri{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIPMU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instVictoria{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUppsala{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instVPI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instWayneState{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instXavier{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instXJTU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYamagata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYonsei{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTYL{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instZZU{\protect\theAffiliationCounter}
\collaboration{The Belle and Belle II Collaborations}
% \author[\instKEK,\instSOKENDAI]{I.~Adachi,} % 2590
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{K.~Adamczyk,} % 2239
  \author[\instPanjab]{L.~Aggarwal,} % 10083
% \author[\instBonn]{P.~Ahlburg,} % 2367
  \author[\instXavier]{H.~Ahmed,} % 11323
% \author[\instKoreaUnivKU]{J.~K.~Ahn,} % 7423
  \author[\instUTokyo]{H.~Aihara,} % 2223
  \author[\instYerevan]{N.~Akopov,} % 9443
  \author[\instNapoliUNIV,\instNapoliINFN]{A.~Aloisio,} % 2194
  \author[\instTabuk]{N.~Althubiti,} % 21524
% \author[\instMPGHLL]{L.~Andricek,} % 2098
% \author[\instBonn]{M.~Angelsmark,} % 13963
  \author[\instIOP]{N.~Anh~Ky,} % 2218
  \author[\instBNL]{D.~M.~Asner,} % 4684
  \author[\instCincinnati]{H.~Atmacan,} % 2538
% \author[\instBINP,\instNSU]{V.~Aulchenko,} % 8183
% \author[\instHSE]{T.~Aushev,} % 3747
  \author[\instKyiv]{V.~Aushev,} % 2155
  \author[\instNagoya]{M.~Aversano,} % 7363
  \author[\instTabuk]{R.~Ayad,} % 3766
% \author[\instTata]{T.~Aziz,} % 3523
  \author[\instIPHC]{V.~Babu,} % 5623
% \author[\instKrakow]{S.~Bacher,} % 2258
  \author[\instKEK]{H.~Bae,} % 10863
  \author[\instLouisville]{N.~K.~Baghel,} % 21505
  \author[\instIITBhubaneswar]{S.~Bahinipati,} % 2332
% \author[\instSydney]{A.~M.~Bakich,} % 2115
  \author[\instIJCLab]{P.~Bambade,} % 3003
  \author[\instLouisville]{Sw.~Banerjee,} % 8603
% \author[\instPanjab]{S.~Bansal,} % 5163
% \author[\instKEK]{M.~Barrett,} % 2180
% \author[\instPisaUNIV,\instPisaINFN]{G.~Batignani,} % 6643
  \author[\instIPHC]{J.~Baudot,} % 2562
% \author[\instKarlsruhe]{M.~Bauer,} % 9863
  \author[\instDESY]{A.~Baur,} % 5683
  \author[\instVictoria]{A.~Beaubien,} % 6683
  \author[\instDESY]{F.~Becherer,} % 21623
  \author[\instKarlsruhe]{J.~Becker,} % 5403
% \author[\instIITMadras]{P.~K.~Behera,} % 4204
  \author[\instMississippi]{J.~V.~Bennett,} % 2454
% \author[\instRomaTreINFN]{E.~Bernieri,} % 4483
  \author[\instBonn]{F.~U.~Bernlochner,} % 2282
  \author[\instCPPM]{V.~Bertacchi,} % 2212
  \author[\instHEPHYVienna]{M.~Bertemes,} % 2595
  \author[\instTelAviv]{E.~Bertholet,} % 13163
  \author[\instHawaii]{M.~Bessner,} % 3783
  \author[\instPisaUNIV,\instPisaINFN]{S.~Bettarini,} % 2350
  \author[\instIISER]{V.~Bhardwaj,} % 2228
% \author[\instIITGuwahati]{B.~Bhuyan,} % 2097
  \author[\instTorinoUNIV,\instTorinoINFN]{F.~Bianchi,} % 2564
% \author[\instTUM]{L.~Bierwirth,} % 11723
  \author[\instDESY]{T.~Bilka,} % 2484
% \author[\instLMU]{S.~Bilokin,} % 3623
  \author[\instLouisville]{D.~Biswas,} % 8703
% \author[\instKEK]{T.~Bloomfield,} % 2418
  \author[\instBINP,\instNSU]{A.~Bobrov,} % 2294
  \author[\instSoochow,\instHSE]{D.~Bodrov,} % 9643
% \author[\instDESY]{A.~Bolz,} % 15403
% \author[\instBINP,\instNSU]{A.~Bondar,} % 4643
% \author[\instWayneState]{G.~Bonvicini,} % 2095
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{J.~Borah,} % 7083
  \author[\instTorinoUNIV,\instTorinoINFN]{A.~Boschetti,} % 17683
  \author[\instKrakow]{A.~Bozek,} % 2303
  \author[\instLjubljanaJSI,\instLjubljanaUM]{M.~Bra\v{c}ko,} % 2425
  \author[\instRomaTreINFN]{P.~Branchini,} % 2577
% \author[\instISU]{N.~Brenny,} % 19943
  \author[\instCMU]{R.~A.~Briere,} % 2584
  \author[\instHawaii]{T.~E.~Browder,} % 2560
% \author[\instGoettingen]{Y.~Buch,} % 17323
  \author[\instRomaTreINFN]{A.~Budano,} % 2171
  \author[\instRomaTreUNIV,\instRomaTreINFN]{S.~Bussino,} % 5384
% \author[\instFrascati]{A.~Calcaterra,} % 19163
% \author[\instMississippi]{Q.~Campagna,} % 21563
  \author[\instNapoliUNIV,\instNapoliINFN]{M.~Campajola,} % 5223
  \author[\instDESY]{L.~Cao,} % 2099
  \author[\instPisaUNIV,\instPisaINFN]{G.~Casarosa,} % 2491
  \author[\instPerugiaUNIV,\instPerugiaINFN]{C.~Cecchi,} % 2433
  \author[\instIPHC]{J.~Cerasoli,} % 20746
  \author[\instFuJen]{M.-C.~Chang,} % 2827
  \author[\instNTUTaiwan]{P.~Chang,} % 2542
% \author[\instDESY]{R.~Cheaib,} % 2208
  \author[\instSydney]{P.~Cheema,} % 15264
% \author[\instMPP]{V.~Chekelian,} % 2167
% \author[\instISU]{C.~Chen,} % 12803
% \author[\instJLU]{Y.~Q.~Chen,} % 16264
% \author[\instNTUTaiwan]{Y.-T.~Chen,} % 2884
  \author[\instHanyang]{B.~G.~Cheon,} % 2173
  \author[\instBINP]{K.~Chilikin,} % 2308
  \author[\instChiangMai]{K.~Chirapatpimol,} % 10803
  \author[\instHanyang]{H.-E.~Cho,} % 2182
  \author[\instKISTI]{K.~Cho,} % 2516
  \author[\instYonsei]{S.-J.~Cho,} % 2723
  \author[\instCAU]{S.-K.~Choi,} % 2364
  \author[\instISU]{S.~Choudhury,} % 2206
% \author[\instMcGill]{K.~Chu,} % 5203
% \author[\instWayneState]{D.~Cinabro,} % 2092
  \author[\instISU]{J.~Cochran,} % 12604
  \author[\instPisaUNIV,\instPisaINFN]{L.~Corona,} % 3944
% \author[\instMississippi]{L.~M.~Cremaldi,} % 2276
  \author[\instSEU]{J.~X.~Cui,} % 8863
% \author[\instTokyoMetropolitan]{T.~Czank,} % 2254
% \author[\instMNITJaipur]{S.~Das,} % 9163
% \author[\instDESY]{F.~Dattola,} % 3745
  \author[\instCinvestavIPN]{E.~De~La~Cruz-Burelo,} % 2359
  \author[\instAdelaide]{S.~A.~De~La~Motte,} % 2128
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{G.~de~Marino,} % 8364
  \author[\instNapoliUNIV,\instNapoliINFN]{G.~De~Nardo,} % 2459
% \author[\instUBC]{M.~De~Nuccio,} % 2610
  \author[\instKarlsruhe]{G.~De~Pietro,} % 2528
  \author[\instFrascati]{R.~de~Sangro,} % 2524
% \author[\instBonn]{B.~Deschamps,} % 2671
  \author[\instTorinoUNIV,\instTorinoINFN]{M.~Destefanis,} % 2594
% \author[\instKEK]{S.~Dey,} % 5023
% \author[\instCinvestavIPN]{A.~De~Yta-Hernandez,} % 2104
  \author[\instIITHyderabad]{R.~Dhamija,} % 9465
  \author[\instBNL]{A.~Di~Canto,} % 10963
  \author[\instNapoliUNIV,\instNapoliINFN]{F.~Di~Capua,} % 2065
  \author[\instBonn]{J.~Dingfelder,} % 2151
  \author[\instPrague]{Z.~Dole\v{z}al,} % 2319
% \author[\instUAS]{I.~Dom\'{\i}nguez~Jim\'{e}nez,} % 2191
  \author[\instITAR]{T.~V.~Dong,} % 2215
  \author[\instTriesteINFN]{M.~Dorigo,} % 12543
% \author[\instHEPHYVienna]{D.~Dorner,} % 13564
% \author[\instGiessen]{K.~Dort,} % 5583
% \author[\instMelbourne]{D.~Dossett,} % 2574
% \author[\instDESY]{S.~Dreyer,} % 12823
  \author[\instHawaii]{S.~Dubey,} % 11063
% \author[\instBonn]{S.~Duell,} % 2344
  \author[\instTUM]{K.~Dugic,} % 11103
  \author[\instIPHC]{G.~Dujany,} % 9703
  \author[\instKarlsruhe]{P.~Ecker,} % 5563
% \author[\instBonn]{M.~Eliachevitch,} % 2725
  \author[\instBINP,\instNSU]{D.~Epifanov,} % 2551
  \author[\instKarlsruhe]{J.~Eppelt,} % 19723
% \author[\instDESY]{Y.~Fan,} % 21303
  \author[\instHEPHYVienna]{P.~Feichtinger,} % 9843
  \author[\instKarlsruhe]{T.~Ferber,} % 2482
% \author[\instMelbourne]{D.~Ferlewicz,} % 2073
  \author[\instKEK]{T.~Fillinger,} % 9803
  \author[\instIPHC]{C.~Finck,} % 15803
  \author[\instFrascati]{G.~Finocchiaro,} % 2400
% \author[\instHeidelberg]{P.~Fischer,} % 2141
% \author[\instHawaii]{K.~Flood,} % 12103
  \author[\instMcGill]{A.~Fodor,} % 2312
  \author[\instPisaUNIV,\instPisaINFN]{F.~Forti,} % 2432
% \author[\instGoettingen]{A.~Frey,} % 2150
% \author[\instHEPHYVienna]{M.~Friedl,} % 2442
  \author[\instPNNL]{B.~G.~Fulsom,} % 2563
  \author[\instPisaINFN]{A.~Gabrielli,} % 13523
% \author[\instBINP,\instNSU]{N.~Gabyshev,} % 2510
  \author[\instDESY]{E.~Ganiev,} % 4623
  \author[\instKEK]{M.~Garcia-Hernandez,} % 4823
  \author[\instCMU]{R.~Garg,} % 2213
% \author[\instBINP,\instNSU]{A.~Garmash,} % 2161
  \author[\instNapoliINFN]{G.~Gaudino,} % 16563
  \author[\instUPES]{V.~Gaur,} % 2413
  \author[\instPadovaUNIV,\instPadovaINFN]{A.~Gaz,} % 2181
% \author[\instGoettingen]{U.~Gebauer,} % 2174
  \author[\instDESY]{A.~Gellrich,} % 2480
  \author[\instYerevan]{G.~Ghevondyan,} % 9445
  \author[\instTriesteUNIV,\instTriesteINFN]{D.~Ghosh,} % 11923
  \author[\instYerevan]{H.~Ghumaryan,} % 19543
  \author[\instBonn]{G.~Giakoustidis,} % 13723
  \author[\instNapoliUNIV,\instNapoliINFN]{R.~Giordano,} % 2103
  \author[\instIITHyderabad]{A.~Giri,} % 2106
  \author[\instIPHC]{P.~Gironella~Gironell,} % 25443
% \author[\instDESY]{A.~Glazov,} % 2473
  \author[\instTriesteINFN]{B.~Gobbo,} % 2109
  \author[\instSAlabama]{R.~Godang,} % 2449
  \author[\instKyiv]{O.~Gogota,} % 2334
  \author[\instKarlsruhe]{P.~Goldenzweig,} % 2345
% \author[\instNovaGorica,\instLjubljanaJSI]{B.~Golob,} % 3703
% \author[\instUSTC]{G.~Gong,} % 2727
% \author[\instAdelaide]{P.~Grace,} % 9563
  \author[\instMainz]{W.~Gradl,} % 2570
% \author[\instDESY]{M.~Graf-Schreiber,} % 2730
% \author[\instVictoria]{T.~Grammatico,} % 20623
% \author[\instBonn]{S.~Granderath,} % 8383
  \author[\instRomaTreINFN]{E.~Graziani,} % 2342
% \author[\instTUM]{D.~Greenwald,} % 2686
  \author[\instPrague]{Z.~Gruberov\'{a},} % 8824
% \author[\instPittsburgh]{T.~Gu,} % 14283
  \author[\instCincinnati]{Y.~Guan,} % 2514
  \author[\instBINP,\instNSU]{K.~Gudkova,} % 10504
  \author[\instKarlsruhe]{I.~Haide,} % 14824
% \author[\instHEPHYVienna]{H.~Haigh,} % 16744
% \author[\instTata]{S.~Halder,} % 4743
  \author[\instDESY]{Y.~Han,} % 19663
% \author[\instKEK,\instSOKENDAI]{K.~Hara,} % 2462
  \author[\instKEK,\instSOKENDAI]{T.~Hara,} % 2523
% \author[\instAdelaide]{C.~Harris,} % 21383
% \author[\instHawaii]{O.~Hartbrich,} % 2158
% \author[\instNiigata]{K.~Hayasaka,} % 2330
  \author[\instNaraWu]{H.~Hayashii,} % 2455
  \author[\instMPP]{S.~Hazra,} % 7663
  \author[\instUBC,\instIPP]{C.~Hearty,} % 2450
% \author[\instBonn]{M.~T.~Hedges,} % 2265
  \author[\instKarlsruhe]{A.~Heidelbach,} % 16923
  \author[\instCinvestavIPN,\instConacyt]{I.~Heredia~de~la~Cruz,} % 2559
% \author[\instBNL]{M.~Hern\'{a}ndez~Villanueva,} % 2466
  \author[\instIPMU]{T.~Higuchi,} % 2485
% \author[\instNagoya]{H.~Hirata,} % 2070
  \author[\instMainz]{M.~Hoek,} % 2101
  \author[\instMelbourne]{M.~Hohmann,} % 2077
  \author[\instDESY]{R.~Hoppe,} % 23383
  \author[\instHEPHYVienna]{P.~Horak,} % 13583
% \author[\instRCNP]{T.~Hotta,} % 2084
  \author[\instSydney]{C.-L.~Hsu,} % 2299
% \author[\instSydney]{A.~Huang,} % 14223
% \author[\instNTUTaiwan]{K.~Huang,} % 2389
  \author[\instDESY]{T.~Humair,} % 10643
  \author[\instNagoya,\instNagoyaKMI,\instKEK]{T.~Iijima,} % 2446
% \author[\instNagoya,\instKEK]{K.~Inami,} % 2323
% \author[\instHEPHYVienna]{G.~Inguglia,} % 2500
  \author[\instIITHyderabad]{N.~Ipsita,} % 12223
  \author[\instKEK,\instSOKENDAI]{A.~Ishikawa,} % 2281
% \author[\instKEK]{S.~Ito,} % 17463
  \author[\instKEK,\instSOKENDAI]{R.~Itoh,} % 2487
  \author[\instOsakaMetropolitan]{M.~Iwasaki,} % 2360
% \author[\instKEK]{Y.~Iwasaki,} % 2229
% \author[\instTokyoMetropolitan]{S.~Iwata,} % 4323
  \author[\instAdelaide]{P.~Jackson,} % 2255
  \author[\instIndiana]{W.~W.~Jacobs,} % 2322
% \author[\instBNL]{D.~E.~Jaffe,} % 3663
  \author[\instGyeongsang]{E.-J.~Jang,} % 6744
  \author[\instHNU]{Q.~P.~Ji,} % 16243
  \author[\instSEU]{S.~Jia,} % 2457
  \author[\instBNL]{Y.~Jin,} % 2105
  \author[\instIITMadras]{A.~Johnson,} % 16143
  \author[\instChonnam]{K.~K.~Joo,} % 4224
  \author[\instBonn]{H.~Junkerkalefeld,} % 12963
% \author[\instKyiv]{I.~Kadenko,} % 3843
% \author[\instTokyoMetropolitan]{H.~Kakuno,} % 2391
% \author[\instKrakow]{M.~Kaleta,} % 5603
% \author[\instIITGuwahati]{D.~Kalita,} % 2220
% \author[\instHEPHYVienna]{A.~B.~Kaliyar,} % 7344
  \author[\instPadovaINFN]{J.~Kandra,} % 2541
  \author[\instIPMU]{K.~H.~Kang,} % 2283
  \author[\instISU]{S.~Kang,} % 12683
% \author[\instKrakow]{P.~Kapusta,} % 6663
  \author[\instYerevan]{G.~Karyan,} % 2550
% \author[\instNagoya,\instNagoyaKMI]{Y.~Kato,} % 2549
% \author[\instChiba]{H.~Kawai,} % 4344
  \author[\instKitasato]{T.~Kawasaki,} % 4363
  \author[\instMainz]{F.~Keil,} % 19523
  \author[\instHawaii]{C.~Ketter,} % 2236
% \author[\instBonn]{M.~Khan,} % 15644
  \author[\instMPP]{C.~Kiesling,} % 2168
% \author[\instYonsei]{C.~Kim,} % 20503
  \author[\instHanyang]{C.-H.~Kim,} % 2358
  \author[\instSoongsil]{D.~Y.~Kim,} % 2315
  \author[\instYonsei]{J.-Y.~Kim,} % 20223
  \author[\instKISTI]{K.-H.~Kim,} % 2118
  \author[\instYonsei]{Y.-K.~Kim,} % 2379
% \author[\instKoreaUnivKU]{Y.~J.~Kim,} % 2403
% \author[\instVPI,\instKEK]{H.~Kindo,} % 2195
  \author[\instCincinnati]{K.~Kinoshita,} % 2318
% \author[\instDESY]{C.~Kleinwort,} % 2499
  \author[\instPrague]{P.~Kody\v{s},} % 2407
  \author[\instKEK]{T.~Koga,} % 6963
  \author[\instHawaii]{S.~Kohani,} % 9143
  \author[\instNagoya]{K.~Kojima,} % 6363
% \author[\instKitasato]{T.~Konno,} % 2490
% \author[\instHawaii]{H.~Korandla,} % 18783
  \author[\instBINP,\instNSU]{A.~Korobov,} % 4185
  \author[\instLjubljanaJSI,\instLjubljanaUM]{S.~Korpar,} % 2475
% \author[\instIJCLab]{E.~Kou,} % 3765
  \author[\instBINP,\instNSU]{E.~Kovalenko,} % 3884
  \author[\instVictoria]{R.~Kowalewski,} % 2293
% \author[\instMPP]{T.~M.~G.~Kraetzschmar,} % 7543
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{P.~Kri\v{z}an,} % 2474
% \author[\instMississippi]{R.~Kroeger,} % 2242
  \author[\instBINP,\instNSU]{P.~Krokovny,} % 2575
% \author[\instGiessen]{W.~Kuehn,} % 2534
% \author[\instDESY,\instLMU]{M.~K\"{u}nzel,} % 2139
  \author[\instLMU]{T.~Kuhr,} % 2486
  \author[\instLMU]{Y.~Kulii,} % 9823
% \author[\instIITGuwahati]{D.~Kumar,} % 7223
% \author[\instIITJodhpur]{J.~Kumar,} % 6464
% \author[\instIISER]{M.~Kumar,} % 2744
  \author[\instPanjabPAU]{R.~Kumar,} % 2189
  \author[\instMississippi]{K.~Kumara,} % 2257
% \author[\instTokyoMetropolitan]{T.~Kumita,} % 4083
  \author[\instKEK]{T.~Kunigo,} % 10104
% \author[\instNaraWu]{A.~Kusudo,} % 14623
  \author[\instBINP,\instNSU]{A.~Kuzmin,} % 2520
% \author[\instPrague]{P.~Kvasni\v{c}ka,} % 2184
  \author[\instYonsei]{Y.-J.~Kwon,} % 2231
% \author[\instPadovaINFN]{S.~Lacaprara,} % 2447
  \author[\instKEK]{Y.-T.~Lai,} % 2066
  \author[\instMNITJaipur]{K.~Lalwani,} % 2142
  \author[\instVPI]{T.~Lam,} % 2729
% \author[\instTriesteINFN]{L.~Lanceri,} % 2540
% \author[\instGiessen]{J.~S.~Lange,} % 2277
  \author[\instKEK]{T.~S.~Lau,} % 19803
  \author[\instUppsala]{M.~Laurenza,} % 10223
% \author[\instCPPM]{K.~Lautenbach,} % 2102
% \author[\instBNL]{P.~J.~Laycock,} % 7683
  \author[\instUBC]{R.~Leboucher,} % 14083
  \author[\instIJCLab]{F.~R.~Le~Diberder,} % 3267
  \author[\instSKKU]{M.~J.~Lee,} % 21803
% \author[\instMPP]{P.~Leitl,} % 2414
  \author[\instCPPM]{C.~Lemettais,} % 22704
  \author[\instDESY,\instHamburg]{P.~Leo,} % 19823
% \author[\instKEK]{D.~Levit,} % 2507
% \author[\instHawaii]{P.~M.~Lewis,} % 2582
  \author[\instLNNU]{C.~Li,} % 2325
  \author[\instCincinnati]{L.~K.~Li,} % 3263
  \author[\instIHEPChina]{Q.~M.~Li,} % 22943
% \author[\instFudan]{S.~X.~Li,} % 2377
  \author[\instBeihang]{W.~Z.~Li,} % 19703
  \author[\instFudan]{Y.~Li,} % 8083
  \author[\instXJTU]{Y.~B.~Li,} % 2573
  \author[\instIHEPChina]{Y.~P.~Liao,} % 24303
  \author[\instIITMadras]{J.~Libby,} % 2262
% \author[\instLMU]{K.~Lieret,} % 2268
  \author[\instNTUTaiwan]{J.~Lin,} % 2401
% \author[\instHiroshima]{Z.~Liptak,} % 3565
  \author[\instJLU]{M.~H.~Liu,} % 15244
  \author[\instHawaii]{Q.~Y.~Liu,} % 7045
  \author[\instKEK,\instSOKENDAI]{Y.~Liu,} % 16223
% \author[\instIHEPChina]{Z.~A.~Liu,} % 3283
  \author[\instShandong]{Z.~Q.~Liu,} % 11303
  \author[\instWayneState,\instKEK]{D.~Liventsev,} % 2578
  \author[\instManitoba]{S.~Longo,} % 2396
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{A.~Lozar,} % 12423
  \author[\instLMU]{T.~Lueck,} % 2406
% \author[\instFudan]{T.~Luo,} % 3268
  \author[\instBonn]{C.~Lyu,} % 12484
% \author[\instRIKENMSL]{Y.~Ma,} % 16883
  \author[\instTorinoUNIV,\instTorinoINFN]{M.~Maggiora,} % 5343
  \author[\instIITHyderabad]{S.~P.~Maharana,} % 19083
  \author[\instTorinoINFN]{R.~Maiti,} % 12043
% \author[\instIITBhubaneswar]{S.~Maity,} % 2985
  \author[\instCPPM]{G.~Mancinelli,} % 20743
  \author[\instBNL]{R.~Manfredi,} % 10303
  \author[\instPerugiaINFN]{E.~Manoni,} % 2305
% \author[\instBonn]{A.~C.~Manthei,} % 15023
  \author[\instTriesteUNIV,\instTriesteINFN]{M.~Mantovano,} % 19783
  \author[\instMelbourne]{D.~Marcantonio,} % 11163
  \author[\instTorinoUNIV,\instTorinoINFN]{S.~Marcello,} % 4223
  \author[\instIFIC]{C.~Marinas,} % 2133
% \author[\instIPHC]{L.~Martel,} % 13503
  \author[\instRomaTreINFN]{C.~Martellini,} % 16983
  \author[\instIJCLab]{A.~Martens,} % 13823
  \author[\instDESY]{A.~Martini,} % 2336
  \author[\instDESY]{T.~Martinov,} % 19463
  \author[\instPisaUNIV,\instPisaINFN]{L.~Massaccesi,} % 16323
% \author[\instRCNP,\instEri]{M.~Masuda,} % 2238
% \author[\instUOM]{T.~Matsuda,} % 5543
% \author[\instKEK,\instNagoya]{K.~Matsuoka,} % 2316
% \author[\instBINP,\instNSU]{D.~Matvienko,} % 2351
  \author[\instIITGuwahati]{S.~K.~Maurya,} % 9763
% \author[\instIJCLab]{F.~Mawas,} % 20943
  \author[\instUBC]{J.~A.~McKenna,} % 2392
% \author[\instMPP]{F.~Meggendorfer,} % 7103
  \author[\instTata]{R.~Mehta,} % 15203
  \author[\instDuke]{F.~Meier,} % 3103
  \author[\instNapoliUNIV,\instNapoliINFN]{M.~Merola,} % 2456
% \author[\instBonn]{F.~Metzner,} % 2296
% \author[\instMelbourne]{M.~Milesi,} % 5443
  \author[\instVictoria]{C.~Miller,} % 2273
  \author[\instNapoliINFN]{M.~Mirra,} % 14744
  \author[\instISU]{S.~Mitra,} % 19944
% \author[\instNaraWu,\instKEK]{K.~Miyabayashi,} % 2327
% \author[\instKEK,\instSOKENDAI]{H.~Miyake,} % 2452
% \author[\instIJCLab]{R.~Mizuk,} % 2483
% \author[\instTata]{G.~B.~Mohanty,} % 2278
% \author[\instCinvestavIPN]{N.~Molina-Gonzalez,} % 8004
  \author[\instPisaUNIV,\instPisaINFN]{S.~Mondal,} % 19743
  \author[\instPerugiaUNIV,\instPerugiaINFN]{S.~Moneta,} % 13303
% \author[\instKoreaUnivKU]{H.~Moon,} % 2304
  \author[\instMPP]{H.-G.~Moser,} % 2120
% \author[\instHEPHYVienna]{M.~Mrvar,} % 2527
% \author[\instKarlsruhe]{Th.~Muller,} % 2165
% \author[\instTorinoINFN]{R.~Mussa,} % 2372
  \author[\instKEK,\instSOKENDAI]{I.~Nakamura,} % 3463
% \author[\instKEK,\instSOKENDAI]{K.~R.~Nakamura,} % 2417
% \author[\instOsakaMetropolitan]{E.~Nakano,} % 2554
  \author[\instKEK,\instSOKENDAI]{M.~Nakao,} % 2498
% \author[\instKEK,\instSOKENDAI]{H.~Nakayama,} % 2232
% \author[\instNTUTaiwan]{H.~Nakazawa,} % 2335
% \author[\instKEK]{Y.~Nakazawa,} % 17383
% \author[\instDESY]{A.~Narimani~Charan,} % 10143
  \author[\instKyotoU]{M.~Naruki,} % 4583
  \author[\instKrakow]{Z.~Natkaniec,} % 3923
  \author[\instBNL]{A.~Natochii,} % 12063
% \author[\instIITHyderabad]{L.~Nayak,} % 9464
  \author[\instIISc]{M.~Nayak,} % 2371
  \author[\instYerevan]{G.~Nazaryan,} % 9523
  \author[\instKarlsruhe]{M.~Neu,} % 23304
% \author[\instDESY]{C.~Niebuhr,} % 2477
% \author[\instKSU]{M.~Niiyama,} % 2063
% \author[\instMPGHLL]{J.~Ninkovic,} % 2386
% \author[\instBNL]{N.~K.~Nisar,} % 2522
  \author[\instKEK,\instSOKENDAI,\instNiigata]{S.~Nishida,} % 2571
% \author[\instHawaii]{K.~Nishimura,} % 3063
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{A.~Novosel,} % 15523
  \author[\instToho]{S.~Ogawa,} % 6263
% \author[\instNagoya]{R.~Okubo,} % 10743
% \author[\instCAU]{S.~L.~Olsen,} % 4563
% \author[\instKyiv]{Y.~Onishchuk,} % 2157
  \author[\instNiigata]{H.~Ono,} % 2160
% \author[\instUTokyo]{Y.~Onuki,} % 2331
% \author[\instIJCLab]{P.~Oskin,} % 9623
  \author[\instUTokyo]{F.~Otani,} % 16244
  \author[\instCMU]{E.~R.~Oxford,} % 6943
% \author[\instKEK,\instSOKENDAI]{H.~Ozaki,} % 2984
% \author[\instHSE]{P.~Pakhlov,} % 2221
  \author[\instHSE]{G.~Pakhlova,} % 2188
% \author[\instPisaUNIV,\instPisaINFN]{A.~Paladino,} % 2435
% \author[\instPittsburgh]{T.~Pang,} % 2114
% \author[\instMississippi]{A.~Panta,} % 7943
  \author[\instPisaUNIV,\instPisaINFN]{E.~Paoloni,} % 2488
  \author[\instNapoliINFN]{S.~Pardi,} % 2532
% \author[\instDuke]{K.~Parham,} % 10684
  \author[\instKyungpook]{H.~Park,} % 2284
  \author[\instUTokyo]{J.~Park,} % 18203
  \author[\instKISTI]{K.~Park,} % 12243
  \author[\instKEK]{S.-H.~Park,} % 2509
% \author[\instBonn]{B.~Paschen,} % 2159
  \author[\instRomaTreINFN]{A.~Passeri,} % 2116
% \author[\instLouisville]{S.~Patra,} % 3123
% \author[\instTUM]{S.~Paul,} % 2131
  \author[\instLuther]{T.~K.~Pedlar,} % 2421
  \author[\instFrascati]{I.~Peruzzi,} % 2253
% \author[\instHawaii]{R.~Peschke,} % 7123
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{R.~Pestotnik,} % 2476
% \author[\instMelbourne]{F.~Pham,} % 2963
  \author[\instFrascati]{M.~Piccolo,} % 2147
  \author[\instVPI]{L.~E.~Piilonen,} % 2346
% \author[\instTorinoUNIV,\instTorinoINFN]{G.~Pinna~Angioni,} % 13363
% \author[\instUAS]{P.~L.~M.~Podesta-Lerma,} % 2266
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{T.~Podobnik,} % 11223
  \author[\instMississippi]{S.~Pokharel,} % 12283
% \author[\instCPPM]{L.~Polat,} % 9783
% \author[\instTelAviv,\instHSE]{V.~Popov,} % 2096
  \author[\instKEK]{C.~Praz,} % 2726
  \author[\instISU]{S.~Prell,} % 12743
  \author[\instGiessen]{E.~Prencipe,} % 2219
  \author[\instBonn]{M.~T.~Prim,} % 2501
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{I.~Prudiiev,} % 19383
% \author[\instSCarolina]{M.~V.~Purohit,} % 2196
  \author[\instHawaii]{H.~Purwar,} % 12363
% \author[\instDESY]{N.~Rad,} % 11683
  \author[\instHEPHYVienna]{P.~Rados,} % 7383
  \author[\instHEPHYVienna]{G.~Raeuber,} % 18143
  \author[\instTriesteUNIV,\instTriesteINFN]{S.~Raiz,} % 13003
  \author[\instGoettingen]{N.~Rauls,} % 11603
% \author[\instTata]{K.~Ravindran,} % 22503
  \author[\instMPP]{M.~Reif,} % 8043
  \author[\instGiessen]{S.~Reiter,} % 2248
  \author[\instBINP,\instNSU]{M.~Remnev,} % 2785
  \author[\instKarlsruhe]{L.~Reuter,} % 16403
  \author[\instIPHC]{I.~Ripp-Baudot,} % 2469
% \author[\instHeidelberg]{M.~Ritzert,} % 2526
  \author[\instPisaUNIV,\instPisaINFN]{G.~Rizzo,} % 2579
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{L.~B.~Rizzuto,} % 3746
% \author[\instUofA,\instIPP]{S.~H.~Robertson,} % 2471
% \author[\instMelbourne]{P.~Rocchetti,} % 13763
% \author[\instUAS]{D.~Rodr\'{i}guez~P\'{e}rez,} % 2176
  \author[\instDESY]{M.~Roehrken,} % 11883
  \author[\instVictoria,\instIPP]{J.~M.~Roney,} % 2244
% \author[\instSCarolina]{C.~Rosenfeld,} % 2082
  \author[\instDESY]{A.~Rostomyan,} % 2481
  \author[\instDESY]{N.~Rout,} % 2965
% \author[\instKrakow]{M.~Rozanska,} % 2205
% \author[\instNapoliUNIV,\instNapoliINFN]{G.~Russo,} % 2388
% \author[\instISU]{D.~Sahoo,} % 2110
  \author[\instKEK,\instSOKENDAI]{Y.~Sakai,} % 2175
  \author[\instMississippi]{D.~A.~Sanders,} % 2458
  \author[\instIITHyderabad]{S.~Sandilya,} % 2286
% \author[\instCincinnati]{A.~Sangal,} % 2384
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{L.~Santelj,} % 2185
% \author[\instIPHC]{C.~Santos,} % 23743
% \author[\instPadovaUNIV,\instPadovaINFN]{P.~Sartori,} % 4523
% \author[\instKEK]{Y.~Sato,} % 5243
  \author[\instPittsburgh]{V.~Savinov,} % 2292
  \author[\instUppsala]{B.~Scavino,} % 2518
% \author[\instLMU,\instMPP]{C.~Schmitt,} % 15063
% \author[\instBonn]{J.~Schmitz,} % 12863
  \author[\instDuke]{S.~Schneider,} % 16803
  \author[\instKarlsruhe]{M.~Schnepf,} % 15683
% \author[\instHawaii]{J.~Schueler,} % 2824
  \author[\instHEPHYVienna]{C.~Schwanda,} % 2108
  \author[\instCincinnati]{A.~J.~Schwartz,} % 2162
% \author[\instGoettingen]{B.~Schwenker,} % 2405
% \author[\instGoettingen]{M.~Schwickardi,} % 14743
  \author[\instNiigata]{Y.~Seino,} % 2517
  \author[\instRomaTreINFN]{A.~Selce,} % 9043
  \author[\instYamagata]{K.~Senyo,} % 2987
  \author[\instCPPM]{J.~Serrano,} % 12124
  \author[\instMelbourne]{M.~E.~Sevior,} % 2328
  \author[\instMainz]{C.~Sfienti,} % 2214
  \author[\instHUNNU]{W.~Shan,} % 11943
  \author[\instMNITJaipur]{C.~Sharma,} % 11584
% \author[\instHawaii]{V.~Shebalin,} % 2339
% \author[\instFudan]{C.~P.~Shen,} % 2464
  \author[\instUTokyo]{X.~D.~Shi,} % 18843
% \author[\instToho]{H.~Shibuya,} % 2234
  \author[\instMcGill]{T.~Shillington,} % 7983
  \author[\instUTokyo]{T.~Shimasaki,} % 16263
  \author[\instNTUTaiwan]{J.-G.~Shiu,} % 2412
  \author[\instBINP,\instNSU]{D.~Shtol,} % 9223
  \author[\instBINP,\instNSU]{B.~Shwartz,} % 2122
  \author[\instHawaii]{A.~Sibidanov,} % 2419
  \author[\instKarlsruhe]{F.~Simon,} % 2164
  \author[\instPanjab,\instUPES]{J.~B.~Singh,} % 2903
  \author[\instMPP,\instTUM]{J.~Skorupa,} % 12523
% \author[\instMelbourne]{K.~Smith,} % 2243
  \author[\instVictoria,\instIPP]{R.~J.~Sobie,} % 2472
  \author[\instMainz]{M.~Sobotzik,} % 8604
  \author[\instTelAviv]{A.~Soffer,} % 2217
  \author[\instIHEPRussia]{A.~Sokolov,} % 2521
% \author[\instDESY]{Y.~Soloviev,} % 2479
  \author[\instBINP]{E.~Solovieva,} % 2398
  \author[\instTorinoUNIV,\instTorinoINFN]{S.~Spataro,} % 2117
  \author[\instMainz]{B.~Spruck,} % 2493
  \author[\instJLU]{W.~Song,} % 22863
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{M.~Stari\v{c},} % 2326
  \author[\instIPHC]{P.~Stavroulakis,} % 20643
  \author[\instKarlsruhe]{S.~Stefkova,} % 8783
% \author[\instHawaii]{L.~Stoetzer,} % 19283
% \author[\instVPI]{Z.~S.~Stottler,} % 2267
  \author[\instPadovaUNIV,\instPadovaINFN]{R.~Stroili,} % 2465
  \author[\instPNNL]{J.~Strube,} % 2451
  \author[\instNagoya]{Y.~Sue,} % 2085
% \author[\instUTokyo]{R.~Sugiura,} % 4644
  \author[\instRCNP,\instGifu]{M.~Sumihama,} % 4243
  \author[\instKEK,\instSOKENDAI,\instNaraWu]{K.~Sumisawa,} % 2583
  \author[\instBonn]{W.~Sutcliffe,} % 3784
  \author[\instChula]{N.~Suwonjandee,} % 14063
% \author[\instKEK,\instSOKENDAI]{S.~Y.~Suzuki,} % 2496
  \author[\instDESY]{H.~Svidras,} % 11783
% \author[\instDESY]{M.~Takahashi,} % 2467
  \author[\instSPU,\instJPARC,\instRIKENMSL]{M.~Takizawa,} % 2437
  \author[\instTorinoINFN]{U.~Tamponi,} % 2366
% \author[\instKEK,\instSOKENDAI]{S.~Tanaka,} % 2530
  \author[\instJAEA]{K.~Tanida,} % 3803
% \author[\instUTokyo]{H.~Tanigawa,} % 2237
% \author[\instKEK]{N.~Taniguchi,} % 2285
  \author[\instPisaUNIV,\instPisaINFN]{F.~Tenchini,} % 2546
  \author[\instCPPM]{A.~Thaller,} % 16044
  \author[\instMPP]{O.~Tittel,} % 8663
  \author[\instTata]{R.~Tiwary,} % 10403
% \author[\instTriesteINFN]{D.~Tonelli,} % 4564
  \author[\instPadovaINFN]{E.~Torassa,} % 2556
% \author[\instSydney]{N.~Toutounji,} % 2263
  \author[\instTYL]{K.~Trabelsi,} % 2369
  \author[\instBonn]{I.~Tsaklidis,} % 13443
% \author[\instKEK,\instSOKENDAI]{T.~Tsuboyama,} % 2361
% \author[\instNagoya]{N.~Tsuzuki,} % 2352
% \author[\instTitech]{M.~Uchida,} % 2370
  \author[\instKEK,\instSOKENDAI]{I.~Ueda,} % 2519
% \author[\instKEK,\instSOKENDAI]{S.~Uehara,} % 2586
% \author[\instUTokyo]{Y.~Uematsu,} % 5883
% \author[\instHSE]{T.~Uglov,} % 2252
  \author[\instKarlsruhe]{K.~Unger,} % 9463
  \author[\instHanyang]{Y.~Unno,} % 2420
  \author[\instKEK]{K.~Uno,} % 14963
  \author[\instKEK,\instSOKENDAI]{S.~Uno,} % 2149
  \author[\instMelbourne]{P.~Urquijo,} % 2302
% \author[\instKEK,\instUTokyo,\instSOKENDAI]{Y.~Ushiroda,} % 2317
% \author[\instBINP,\instNSU]{Y.~V.~Usov,} % 5003
  \author[\instHawaii]{S.~E.~Vahsen,} % 2251
  \author[\instMcGill]{R.~van~Tonder,} % 2706
% \author[\instHawaii]{G.~S.~Varner,} % 2119
% \author[\instSydney]{K.~E.~Varvell,} % 2545
  \author[\instISU]{M.~Veronesi,} % 20723
% \author[\instBINP,\instNSU]{A.~Vinokurova,} % 2289
  \author[\instIITHyderabad]{V.~S.~Vismaya,} % 16063
  \author[\instTriesteUNIV,\instTriesteINFN]{L.~Vitale,} % 2415
  \author[\instIFIC]{V.~Vobbilisetti,} % 7364
  \author[\instPerugiaUNIV,\instPerugiaINFN]{R.~Volpe,} % 20183
% \author[\instBINP]{V.~Vorobyev,} % 2298
% \author[\instDuke]{A.~Vossen,} % 2249
% \author[\instMPP,\instTUM]{B.~Wach,} % 8203
% \author[\instKEK]{E.~Waheed,} % 2226
  \author[\instUBC]{M.~Wakai,} % 3583
% \author[\instMcGill]{H.~M.~Wakeling,} % 3664
  \author[\instMPP]{S.~Wallner,} % 20363
% \author[\instMalaya]{W.~Wan~Abdullah,} % 2280
% \author[\instCincinnati]{B.~Wang,} % 2569
% \author[\instNUUTaiwan]{C.~H.~Wang,} % 2224
% \author[\instPittsburgh]{E.~Wang,} % 10983
  \author[\instNTUTaiwan]{M.-Z.~Wang,} % 2074
  \author[\instFudan]{X.~L.~Wang,} % 2076
  \author[\instUTokyo]{Z.~Wang,} % 15743
  \author[\instMcGill]{A.~Warburton,} % 2347
% \author[\instNiigata]{M.~Watanabe,} % 2309
  \author[\instCincinnati]{S.~Watanuki,} % 6843
% \author[\instBonn]{M.~Welsch,} % 7023
% \author[\instTriesteINFN]{O.~Werbycka,} % 6123
  \author[\instDESY]{C.~Wessel,} % 2100
% \author[\instKrakow]{J.~Wiechczynski,} % 2604
% \author[\instGoettingen]{P.~Wieduwilt,} % 2343
% \author[\instMPP]{H.~Windel,} % 2081
% \author[\instKoreaUnivKU]{E.~Won,} % 2410
% \author[\instShandong]{Y.~Xie,} % 20383
  \author[\instSoochow]{X.~P.~Xu,} % 4923
  \author[\instSydney]{B.~D.~Yabsley,} % 3645
  \author[\instKEK]{S.~Yamada,} % 2492
  \author[\instUSTC]{W.~Yan,} % 2094
% \author[\instKoreaUnivKU]{S.~B.~Yang,} % 2374
  \author[\instFlorida]{J.~Yelton,} % 2067
  \author[\instNankai]{J.~H.~Yin,} % 2365
% \author[\instIHEPChina]{Y.~M.~Yook,} % 2453
% \author[\instHawaii]{K.~Yoshihara,} % 12663
% \author[\instLMU]{B.~Yu,} % 15563
  \author[\instIHEPChina]{C.~Z.~Yuan,} % 2088
% \author[\instJLU]{J.~Yuan,} % 23423
% \author[\instNiigata]{Y.~Yusa,} % 2357
  \author[\instRomaTreUNIV,\instRomaTreINFN]{L.~Zani,} % 2529
  \author[\instIPMU]{F.~Zeng,} % 22043
% \author[\instHawaii]{B.~Zhang,} % 11663
% \author[\instIHEPChina]{J.~Z.~Zhang,} % 2349
% \author[\instFudan]{Y.~Zhang,} % 3303
% \author[\instUSTC]{Z.~Zhang,} % 5363
% \author[\instBINP,\instNSU]{V.~Zhilich,} % 4703
  \author[\instFudan]{J.~S.~Zhou,} % 12463
  \author[\instShandong]{Q.~D.~Zhou,} % 7323
% \author[\instLNNU]{X.~Y.~Zhou,} % 2380
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{V.~I.~Zhukova,} % 2387
% \author[\instBINP,\instNSU]{V.~Zhulanov,} % 4983
  \author[\instTriesteINFN]{R.~\v{Z}leb\v{c}\'{i}k} % 13403
\affiliation[\instCPPM]{Aix Marseille Universit\'{e}, CNRS/IN2P3, CPPM, 13288 Marseille, France}
\affiliation[\instYerevan]{Alikhanyan National Science Laboratory, Yerevan 0036, Armenia}
\affiliation[\instGoettingen]{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
\affiliation[\instBeihang]{Beihang University, Beijing 100191, China}
\affiliation[\instBNL]{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\affiliation[\instBINP]{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
\affiliation[\instCMU]{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\affiliation[\instCinvestavIPN]{Centro de Investigacion y de Estudios Avanzados del Instituto Politecnico Nacional, Mexico City 07360, Mexico}
\affiliation[\instPrague]{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
\affiliation[\instChiangMai]{Chiang Mai University, Chiang Mai 50202, Thailand}
%%%\affiliation[\instChiba]{Chiba University, Chiba 263-8522, Japan}
\affiliation[\instChonnam]{Chonnam National University, Gwangju 61186, South Korea}
\affiliation[\instChula]{Chulalongkorn University, Bangkok 10330, Thailand}
\affiliation[\instCAU]{Chung-Ang University, Seoul 06974, South Korea}
\affiliation[\instConacyt]{Consejo Nacional de Ciencia y Tecnolog\'{\i}a, Mexico City 03940, Mexico}
\affiliation[\instDESY]{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\affiliation[\instDuke]{Duke University, Durham, North Carolina 27708, U.S.A.}
\affiliation[\instITAR]{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
\affiliation[\instFuJen]{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\affiliation[\instFudan]{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\affiliation[\instGifu]{Gifu University, Gifu 501-1193, Japan}
\affiliation[\instSOKENDAI]{The Graduate University for Advanced Studies (Sokendai), Tsukuba 305-0801, Japan}
\affiliation[\instMainz]{Institut f\"{u}r Kernphysik, Johannes Gutenberg-Universit\"{a}t Mainz, D-55099 Mainz, Germany}
\affiliation[\instGyeongsang]{Gyeongsang National University, Jinju 52828, South Korea}
\affiliation[\instHanyang]{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
%%%\affiliation[\instHeidelberg]{Heidelberg University, 68131 Mannheim, Germany}
\affiliation[\instHNU]{Henan Normal University, Xinxiang 453007, China}
\affiliation[\instKEK]{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\affiliation[\instJPARC]{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
%%%\affiliation[\instHiroshima]{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530, Japan}
\affiliation[\instHUNNU]{Hunan Normal University, Changsha 410081, China}
\affiliation[\instFrascati]{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy}
\affiliation[\instNapoliINFN]{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\affiliation[\instPadovaINFN]{INFN Sezione di Padova, I-35131 Padova, Italy}
\affiliation[\instPerugiaINFN]{INFN Sezione di Perugia, I-06123 Perugia, Italy}
\affiliation[\instPisaINFN]{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\affiliation[\instRomaTreINFN]{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\affiliation[\instTorinoINFN]{INFN Sezione di Torino, I-10125 Torino, Italy}
\affiliation[\instTriesteINFN]{INFN Sezione di Trieste, I-34127 Trieste, Italy}
\affiliation[\instIISc]{Indian Institute of Science, Bengaluru 560012, India}
\affiliation[\instIISER]{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
\affiliation[\instIITBhubaneswar]{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050, India}
\affiliation[\instIITGuwahati]{Indian Institute of Technology Guwahati, Assam 781039, India}
\affiliation[\instIITHyderabad]{Indian Institute of Technology Hyderabad, Telangana 502285, India}
%%%\affiliation[\instIITJodhpur]{Indian Institute of Technology Jodhpur, Jodhpur 342030, India}
\affiliation[\instIITMadras]{Indian Institute of Technology Madras, Chennai 600036, India}
\affiliation[\instIndiana]{Indiana University, Bloomington, Indiana 47408, U.S.A.}
\affiliation[\instIHEPRussia]{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\affiliation[\instHEPHYVienna]{Institute of High Energy Physics, Vienna 1050, Austria}
\affiliation[\instIHEPChina]{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
\affiliation[\instIPP]{Institute of Particle Physics (Canada), Victoria, British Columbia V8W 2Y2, Canada}
\affiliation[\instIOP]{Institute of Physics, Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}
\affiliation[\instIFIC]{Instituto de Fisica Corpuscular, Paterna 46980, Spain}
\affiliation[\instISU]{Iowa State University, Ames, Iowa 50011, U.S.A.}
\affiliation[\instJAEA]{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
\affiliation[\instJLU]{Jilin University, Changchun 130012, China}
\affiliation[\instKarlsruhe]{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
\affiliation[\instKitasato]{Kitasato University, Sagamihara 252-0373, Japan}
\affiliation[\instKISTI]{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
%%%\affiliation[\instKoreaUnivKU]{Korea University, Seoul 02841, South Korea}
%%%\affiliation[\instKSU]{Kyoto Sangyo University, Kyoto 603-8555, Japan}
\affiliation[\instKyotoU]{Kyoto University, Kyoto 606-8501, Japan}
\affiliation[\instKyungpook]{Kyungpook National University, Daegu 41566, South Korea}
\affiliation[\instLNNU]{Liaoning Normal University, Dalian 116029, China}
\affiliation[\instGiessen]{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
\affiliation[\instLuther]{Luther College, Decorah, Iowa 52101, U.S.A.}
\affiliation[\instMNITJaipur]{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
\affiliation[\instLMU]{Ludwig Maximilians University, 80539 Munich, Germany}
\affiliation[\instMcGill]{McGill University, Montr\'{e}al, Qu\'{e}bec, H3A 2T8, Canada}
\affiliation[\instNagoya]{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
\affiliation[\instNagoyaKMI]{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
%%%\affiliation[\instNNU]{Nanjing Normal University, Nanjing 210023, China}
\affiliation[\instNankai]{Nankai University, Tianjin 300071, China}
\affiliation[\instNaraWu]{Nara Women's University, Nara 630-8506, Japan}
%%%\affiliation[\instUNAM]{National Autonomous University of Mexico, Mexico City, Mexico}
\affiliation[\instHSE]{National Research University Higher School of Economics, Moscow 101000, Russian Federation}
\affiliation[\instNTUTaiwan]{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
%%%\affiliation[\instNUUTaiwan]{National United University, Miao Li 36003, Taiwan}
\affiliation[\instKrakow]{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\affiliation[\instNiigata]{Niigata University, Niigata 950-2181, Japan}
\affiliation[\instNSU]{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
\affiliation[\instOsakaMetropolitan]{Osaka Metropolitan University, Osaka 558-8585, Japan}
\affiliation[\instRCNP]{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\affiliation[\instPNNL]{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
\affiliation[\instPanjab]{Panjab University, Chandigarh 160014, India}
%%%\affiliation[\instPeking]{Peking University, Beijing 100871, China}
\affiliation[\instMPP]{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
%%%\affiliation[\instMPGHLL]{Semiconductor Laboratory of the Max Planck Society, 81739 M\"{u}nchen, Germany}
\affiliation[\instPanjabPAU]{Punjab Agricultural University, Ludhiana 141004, India}
\affiliation[\instRIKENMSL]{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
\affiliation[\instShandong]{Shandong University, Jinan 250100, China}
\affiliation[\instKyiv]{Taras Shevchenko National University of Kiev, Kiev, Ukraine}
\affiliation[\instSPU]{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
\affiliation[\instSoochow]{Soochow University, Suzhou 215006, China}
\affiliation[\instSoongsil]{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978, South Korea}
\affiliation[\instSEU]{Southeast University, Nanjing 211189, China}
\affiliation[\instLjubljanaJSI]{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\affiliation[\instSKKU]{Sungkyunkwan University, Suwon 16419, South Korea}
\affiliation[\instTata]{Tata Institute of Fundamental Research, Mumbai 400005, India}
\affiliation[\instTUM]{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\affiliation[\instTelAviv]{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978, Israel}
\affiliation[\instToho]{Toho University, Funabashi 274-8510, Japan}
%%%\affiliation[\instTitech]{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
%%%\affiliation[\instTokyoMetropolitan]{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
%%%\affiliation[\instUAS]{Universidad Autonoma de Sinaloa, Sinaloa 80000, Mexico}
\affiliation[\instNapoliUNIV]{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\affiliation[\instPadovaUNIV]{Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova, I-35131 Padova, Italy}
\affiliation[\instPerugiaUNIV]{Dipartimento di Fisica, Universit\`{a} di Perugia, I-06123 Perugia, Italy}
\affiliation[\instPisaUNIV]{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
\affiliation[\instRomaTreUNIV]{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\affiliation[\instTorinoUNIV]{Dipartimento di Fisica, Universit\`{a} di Torino, I-10125 Torino, Italy}
\affiliation[\instTriesteUNIV]{Dipartimento di Fisica, Universit\`{a} di Trieste, I-34127 Trieste, Italy}
\affiliation[\instIJCLab]{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\affiliation[\instIPHC]{Universit\'{e} de Strasbourg, CNRS, IPHC, UMR 7178, 67037 Strasbourg, France}
\affiliation[\instAdelaide]{Department of Physics, University of Adelaide, Adelaide, South Australia 5005, Australia}
%%%\affiliation[\instUofA]{University of Alberta, Edmonton, Alberta, T6G 2E1, Canada}
\affiliation[\instBonn]{University of Bonn, 53115 Bonn, Germany}
\affiliation[\instUBC]{University of British Columbia, Vancouver, British Columbia, V6T 1Z1, Canada}
\affiliation[\instCincinnati]{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\affiliation[\instFlorida]{University of Florida, Gainesville, Florida 32611, U.S.A.}
\affiliation[\instHamburg]{University of Hamburg, 20148 Hamburg, Germany}
\affiliation[\instHawaii]{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\affiliation[\instLjubljanaUniLJ]{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\affiliation[\instLouisville]{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
%%%\affiliation[\instMalaya]{National Centre for Particle Physics, University of Malaya, 50603 Kuala Lumpur, Malaysia}
\affiliation[\instManitoba]{University of Manitoba, Winnipeg, Manitoba, R3T 2N2, Canada}
\affiliation[\instLjubljanaUM]{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor, Slovenia}
\affiliation[\instMelbourne]{School of Physics, University of Melbourne, Victoria 3010, Australia}
\affiliation[\instMississippi]{University of Mississippi, University, Mississippi 38677, U.S.A.}
%%%\affiliation[\instUOM]{University of Miyazaki, Miyazaki 889-2192, Japan}
%%%\affiliation[\instNovaGorica]{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\affiliation[\instUPES]{University of Petroleum and Energy Studies, Dehradun 248007, India}
\affiliation[\instPittsburgh]{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
\affiliation[\instUSTC]{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026, China}
\affiliation[\instSAlabama]{University of South Alabama, Mobile, Alabama 36688, U.S.A.}
%%%\affiliation[\instSCarolina]{University of South Carolina, Columbia, South Carolina 29208, U.S.A.}
\affiliation[\instSydney]{School of Physics, University of Sydney, New South Wales 2006, Australia}
\affiliation[\instTabuk]{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\affiliation[\instUTokyo]{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
%%%\affiliation[\instEri]{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
\affiliation[\instIPMU]{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
\affiliation[\instVictoria]{University of Victoria, Victoria, British Columbia, V8W 3P6, Canada}
\affiliation[\instUppsala]{Uppsala University, SE-751 05 Uppsala, Sweden}
\affiliation[\instVPI]{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\affiliation[\instWayneState]{Wayne State University, Detroit, Michigan 48202, U.S.A.}
\affiliation[\instXavier]{St. Francis Xavier University, Antigonish, Nova Scotia, B2G 2W5, Canada}
\affiliation[\instXJTU]{Xi'an Jiaotong University, Xi'an 710049, China}
\affiliation[\instYamagata]{Yamagata University, Yamagata 990-8560, Japan}
\affiliation[\instYonsei]{Yonsei University, Seoul 03722, South Korea}
\affiliation[\instTYL]{Toshiko Yuasa Laboratory, Tsukuba 305-0801, Japan}
%%%\affiliation[\instZZU]{Zhengzhou University, Zhengzhou 450001, China}

